Towards Building Multilingual Language Model for Medicine

The development of open-source, multilingual medical language models can benefit a wide, linguistically diverse audience from different regions. To promote this domain, we present contributions from the following: First, we construct a multilingual medical corpus, containing approximately 25.5B tokens encompassing 6 main languages, termed as MMedC, enabling auto-regressive domain adaptation for general LLMs; Second, to monitor the development of multilingual medical LLMs, we propose a multilingual medical multi-choice question-answering benchmark with rationale, termed as MMedBench; Third, we have assessed a number of open-source large language models (LLMs) on our benchmark, along with those further auto-regressive trained on MMedC. Our final model, MMed-Llama 3, with only 8B parameters, achieves superior performance compared to all other open-source models on both MMedBench and English benchmarks, even rivaling GPT-4. In conclusion, in this work, we present a large-scale corpus, a benchmark and a series of models to support the development of multilingual medical LLMs.

==> content_acl/00_Abstract.tex <==
In this paper, \weidi{we aim to develop an open-source, multilingual language model for medicine, that enables to ...., to our knowledge, this is the first.....}
In general, we present the contribution from the following aspects:
{\em first,} \weidi{we .... multilingual language corpus for medicine,}
{\em second,} \weidi{we .....}
{\em third,} \weidi{we ...}


specifically, we introduce a new open-source multi-lingual medical corpus, named \textbf{MMedC}, leveraging 4 data sources with automatic preprocessing strategies, containing approximately 25B tokens, encompassing 6 main languages, training a new multi-lingual medical language model on it, termed as MMedLM. Additionally, we also propose a new multi-lingual medical QA benchmark, \textbf{MMedB} and evaluate the performance of most existing medical LLMs together with MMedLM. 
In experiment, we carry out thorough ablation study for different data components and our corpus shows great improvement for different base language model backbone. All resources, including code, model weights, and datasets, will be publicly available.

==> content_acl/01_Introduction.tex <==
\section{Introduction}

Recently, large language models~(LLMs) have achieved remarkable success, also for medical domain. In close-source domain, GPT-4~\cite{openai2023gpt4} and MedPalm-2~\cite{Singhal2022LargeLM} show comparable performance to human clinicians, passing the United States Medical Licensing Examination~(USMLE). Meanwhile in open-source domain, latest Llama\ 2~\cite{touvron2023llama} also inspires a series medical specified LLMs~\cite{PMC-LLAMA,MedAlpaca,clinicalnlp-2023-clinical}. Sadly, most of these superior medical LLMs are mainly targeting at English scenarios, greatly delaying them benefiting more people fairly and widely.

% In recent years, the rapid advancement of large language models (LLMs) has garnered significant attention across various fields due to their remarkable achievements, which is true in the medical domain as well. Current research ~\cite{kung2023performance,nori2023capabilities} has demonstrated that OpenAI's large models such as ChatGPT~\cite{chatgpt} and GPT-4~\cite{openai2023gpt4} have successfully passed the UMLSE exam. Sadly, despite models like ChatGPT excelling in specific medical examinations, they are not specifically designed for the medical field. What's more, studies also indicate that ChatGPT performs poorly in non-English medical exams, such as Japanese~\cite{jpn-med-exam_gpt4}, failing to pass these tests. Direct application of these large models in medical contexts might reduce diagnostic accuracy, potentially harming patients.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/overview2.pdf}
    % \vspace{-10pt}
    \caption{Overview. We developed a method to augment language models' medical capabilities across multiple languages. This involved assembling a comprehensive 105GB medical corpus, comprising 25 billion tokens, for extensive pretraining, infusing the model with specialized medical knowledge. To assess the effectiveness of our multilingual models in the medical domain, we created a benchmark consisting of multilingual, multi-choice medical questions, complete with detailed rationales. Comparative evaluations demonstrate that our approach markedly enhances the model's performance, surpassing that of GPT-3.5 in medical contexts}
\end{figure}


% Current efforts have explored numerous methods to adapt general-purpose LLMs to the medical field. Since OpenAI's GPT series is not open-sourced, most medical models are based on open-source models like LLAMA~\cite{touvron2023llama} and GLM~\cite{du2021glm}. ChatDoctor~\cite{ChatDoctor} has collected 100k real-world patient-doctor dialogues and fine-tuned on this data using LLAMA, also building a Knowledge Brain for external retrieval. MedAlpaca~\cite{MedAlpaca} constructed a dataset exceeding 160,000 entries, experimenting with various fine-tuning techniques on the LLAMA model, such as Lora and 8-bit quantization. PMC-LLAMA~\cite{PMC-LLAMA}, in addition to utilizing GPT-4 to build a fine-tuning dataset of 202M tokens, also created approximately 80B tokens of medical pre-training corpora from medical papers and books, surpassing ChatGPT in multiple medical Q\&A benchmarks.

The main and foundation challenge falls in the lack of a large-scale medical multilingual corpora to support LLM training or adaptation. Thus, in this paper, our goal is to systematically construct a method that automatically acquires a vast high-quality medical multilingual corpus. Additionally, a multilingual medical benchmark to comprehensively monitor the performance of LLMs in the medical domain is also missing. So we collect and build a medical multi-lingual benchmark to further validate the performance of different existing LLMs and the effectiveness of our data.

% Specifically, \chaoyi{in data, we ...} \chaoyi{briefly describe our progress}. \chaoyi{in benchmark, we ...}\chaoyi{remember to highlight human rating score to support the metric investigation.}.

Specifically, we collect an extensive multilingual medical corpora called MMedC by extracting medical knowledge from medical ebooks across the world and filtering medical content from world-largest public-accessible, CommonCrawl. We also add some data as a supplement by crawling data from medical website and collecting a few open-source medical datasets. We called our multilingual LLM undergoing domain knowledge enhancement MMedLM. In order to have a better evaluation of models' performance, we release a multilingual medical QA Benchmark composed of 6 languages multiple-choice questions with rationale. We also conduct human rating and correlation analysis to select suitable automatic metrics for rationale evaluation.

% However, most current medical LLMs excel primarily in one language (mainly English), as their base models are often trained in English. Furthermore, due to issues of medical data privacy and acquisition costs, most medical datasets are in English, posing challenges for non-English applications. To address this, our goal is to systematically construct a method that automatically acquire vast high-quality medical corpus, and then applies open-source multilingual models, such as Internlm~\cite{2023internlm}, to the medical field. We fist collect extensive multilingual medical corpora by filtering open-source data and performing OCR on medical e-books from various countries. We find that pre-training models with multilingual medical corpora effectively embeds regional medical knowledge into the models. Additionally, to objectively compare the performance of various models on multilingual medical problems, we create a multilingual medical benchmark by using GPT-4 to explain the options of multiple-choice questions on publicly available medical exam datasets from different countries.

In summary, our contributions are threefold: \textit{first,} We build a multilingual medical-specific large language model with \chaoyi{25.5B} tokens, covering \chaoyi{6} languages. We carry out thorough ablation study on it to show the importance of each part and existing main-stream language models via continually training on it can be further improved on multilingual benchmarks. \textit{Second,} we release a new medical multilingual benchmark for evaluating multilingual medical models. \chaoyi{Beyond commonly multi-choice QA, we also provide explanation reference and human rating scores to support rationale ability analysis and auto-metric design.}\textit{Third,} in experiment, our final model trained on our corpora shows superior performance across different languages, serving as a new multilingual medical pre-trained mutli-lingual LLM.

==> content_acl/02_Background.tex <==
\section{Background}
\subsection{General LLMs}
In the past five years, the emergence of large language models (LLMs) has revolutionized the field of natural language processing. Despite their simple transformer-based architecture~\cite{attentionIsAllYouNeed}, they perform very well as model parameters increase~\cite{scalingLaws}. LLMs first undergo an initial phase of pretraining, where they are exposed to vast and diverse textual datasets~\cite{C4, mC4, PILE, ROOTs, redpajama}, equipping them with a broad understanding of language patterns. Following this, they are subject to a process of finetuning with instructions and input-output pairs~\cite{chung2022scaling, iyer2022opt, wei2021finetuned, ouyang2022training}. The most attractive thing is the generalize capability of LLM, which allows it to have comparable performance with specific models without any further training~\cite{wei2021finetuned, chowdhery2023palm, wang2022super}. With well-designed prompts~\cite{liu2023zero, kim2023cot}, powerful LLMs can perform well on almost all natural language processing tasks.



%These models, characterized by their extensive pretraining on diverse, large-scale corpora, have demonstrated remarkable generalization capabilities. This advancement allows them to match or even surpass the performance of earlier specialized language models without any shot.

% The particular value of LLMs is the zero-shot learning ability, which enables them to tackle various tasks effectively without task-specific training. This capability has led to their widespread adoption, consistently outperforming traditional language models across multiple performance metrics and establishing a new benchmark for state-of-the-art in the field.

\subsection{Multilingual Language Models}
Multilingual language models refer to models capable of handling queries across different languages. This requires multilingual language models to possess a powerful tokenizer suitable for various languages~\cite{schuster2012japanese,sennrich2015neural,kudo2018subword}, and training on multilingual corpora~\cite{mC4, ROOTs, PILE, abadji-etal-2022-towards, nguyen2023culturax}. Given the need for a larger vocabulary, and the imbalance in different language corpus distribution, there remains challenges in multilingual LLMs~\cite{arivazhagan2019massively,lauscher2020zero}. Noteworthy models in this domain include BigScience's BLOOM~\cite{BLOOM} and Shanghai AI Lab's InternLM~\cite{2023internlm}.

\subsection{Medical Language Models}
% Medical language models refer to models that have undergone pretraining or finetuning with instructions on medical corpora. Prior to 2020, most research was based upon Bert, and many medical bert~\cite{bert} models were released, such as Biobert~\cite{biobert}, Pubmedbert~\cite{pubmedbert} and Biolinkbert~\cite{yasunaga-etal-2022-linkbert}. Although there are some differences in the specific implementation, these models all conduct extensive pre-training on medical corpora, followed by fine-tuning for downstream tasks such as classification, summarization, and information extraction. However, these tasks were still quite distant from practical applications, the performance of the model is relatively low. With the advent of open-source large language models, there has been a significant enhancement in the capabilities of language models in terms of inference and knowledge, with model parameters reaching the billion-scale. Owing to the large size of these model parameters, most research has been focused on fine-tuning with instructions using Llama on medical instructions data. Among these open-source medical LLMs, only PMC-llama has undertaken pre-training on medical corpora, infusing medical information into the model during this phase.

Medical language models are language models that have undergone further training on medical domain data. Prior to 2021, most research was based on BERT~\cite{bert}, such as BioBERT~\cite{biobert}, PubMedBERT~\cite{pubmedbert} and BioLinkBERT~\cite{yasunaga-etal-2022-linkbert}. With the advent of open-source large language models, current efforts mainly explore methods to adapt general-purpose LLMs to medical domain. Since OpenAI's GPT series is not open-sourced, most medical LLMs are based on open-source models like LLaMA~\cite{touvron2023llama} and GLM~\cite{du2021glm}. For instance, ChatDoctor~\cite{ChatDoctor} has collected 100k real-world patient-doctor dialogues and finetuned LLaMA on this data using, also building a Knowledge Brain for external retrieval. MedAlpaca~\cite{MedAlpaca} constructed a dataset exceeding 160,000 entries, experimenting with various fine-tuning techniques on LLaMA model, such as Lora and 8-bit quantization. PMC-LLaMA~\cite{PMC-LLAMA}, in addition to utilizing GPT-4 to build a fine-tuning dataset of 202M tokens, also created approximately 80B tokens of medical pretraining corpora from medical papers and books, surpassing GPT-3.5 in multiple medical QA benchmarks.

% The training data for medical applications is primarily divided into two parts: pre-training and fine-tuning with instructions. Since the data needs for fine-tuning is relatively small, it is usually constructed through specific website crawling or manual annotation. Given the vast size of pre-training corpora, the development of an automated pipeline is essential. 
% For medical dataset collection, there exist many excellent QA dataset suitable for instruction finetuning~\cite{PMC-LLAMA}. However, there is always a lack of medical corpus for large scale pretraining. Previous studies typically used public papers from PMC, extracting medical paper abstracts to construct high-quality medical corpora. PMC-LLaMA ~\cite{PMC-LLAMA} also suggested the possibility of obtaining a large volume of high-quality medical corpora through OCR of ebooks. However, as most publicly available papers are in English, this approach predominantly yields English medical literature, and restricts the diversity of the dataset. There is currently a lack of effective work in gathering extensive multilingual medical corpora for tasks requiring multiple languages.

==> content_acl/03_Methodology.tex <==
\section{Methodology}
In this section, we will introduce our methodology in detail. Specifically, in Sec.~\ref{sec:MMedC}, we will discuss the MMedC construction pipeline and data distribution. Then, in Sec.~\ref{sec:MMedB}, we will discuss our new comprehensive multilingual medical benchmark, MMedB, for the evaluation of multilingual medical models.

\subsection{Large-scale Multilingual Medical Corpus}
\label{sec:MMedC}

 % \chaoyi{I think instruction-tuning is the next version and for this version we just claim the following three contributions: 1. the first large-scale medical-wise multi-linguage corpus. 2. Propose a benchmark covering diverse languages. 3. do ablation on the pre-training data source} \chaoyi{oh, We can also use the corpurses to train a BERT-wise and T-5-wise(this is more like an ablation on training style compared with only-autoregressive) model and similarly testing them on our benchmark so that we can claim we also provide a medical multilingual model zoo for different use cases.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/data_construction.pdf}
    % \vspace{-10pt}
    \caption{MMedC construction. The data mainly from 4 source and consists of 6 languages. Ratio of different data is shown in as the width of the band.}
    \label{fig:data_construction}
\end{figure}

We herein develop a new large-scale multilingual medical corpus, \textbf{MMedC}, to help enrich LLMs with medical domain-specific knowledge across different cultures and countries. In detail, we explore to establish MMedC from four primary sources, \emph{i.e.}, medical filtering-based data from CommonCrawl~\cite{commoncrawl}, medical ebooks, medical websites, and different open-source datasets as depicted in Figure~\ref{fig:data_construction}. Generally, as a result, MMedC contains approximately \textbf{105GB} of data, encompassing over \textbf{25B} tokens, covering \textbf{6 main languages} in total. Next, we will introduce the data collection progress from the four sources respectively and give a bird view on the final data distributions.

% We constructed \textbf{MMedC}, a large-scale multilingual medical-wise corpus, filled with medical domain knowledge across global wide. We constructed the dataset from four sources, as shown in Figure~\ref{fig:data_construction}, The first source involves extracting medical content from CommonCrawl, one of the largest publicly available datasets of web-crawled data. The second source involves the collecting medical ebooks in various languages, which are subsequently converted into text using OCR (Optical Character Recognition) technology. The dataset also involves some articles crawled from medical-related websites in different countries. what's more, we also collect some excellent existing multilingual datasets as a supplement. Consequently, MMedC encompasses approximately 105GB of data, comprising a total of over 25 billion tokens.

% \chaoyi{We need to define a level to classify different datasoruce.}

\subsubsection{Filtering-based Data} 
\label{sec:filtering_based_data}

Compared to the medical-specific field, the general NLP community has already accumulated a vast amount of corpora, \emph{e.g.}, CommonCrawl, which monthly captures billions of web pages and has going on for years. While it's true that medical-related content might represent only a small fraction of this vast dataset, given its enormous scale, we believe this is still a great treasure for establishing a large-scale medical-specific corpus with suitable auto-filtering methods.

% To the best of our knowledge, the largest open-source corpus in the world is CommonCrawl,  The data volume of CommonCrawl is staggering, reaching hundreds of terabytes, but the data contains content on various topics, some of which are even garbled or harmful. Our goal is to filter the medical-related corpus of relatively high quality.

%  Based on these cleaned data, we further create a pipeline to extract medically relevant text from these vast corpora.

\chaoyi{put the following into related work named as ``Corpus COnstruction'' or something with similar meanings.} \pengcheng{Done}Thankfully, there have been many excellent work making efforts to clean the CommonCrawl, such as OSCAR~\cite{abadji-etal-2022-towards}, CulturaX~\cite{nguyen2023culturax}. They have filtered out the noise and harmful data from CommonCrawl, and release a cleaned version of data.
% We extracted medical content through the application of Metric-Based Filtering. Given the extensive volume of data involved, exceeding 4TB, this straightforward, rule-based approach proves highly efficient. We first compiled a list of high-frequent used medical terms. Considering the linguistic nuances across different languages, we individually identified 200 medical-relevant terms for each language, spanning the domains of medicine, pharmacy, and medical biology. Together with these terms, we established two key metrics:

Specifically, we start with the CulturaX~\cite{nguyen2023culturax} dataset, which is a further multilingual separated and cleaned version of CommonCrawl with \chaoyi{6.3 Trillion} tokens. We propose a new \textbf{rule-based filtering} pipeline to extract medical content. First, we meticulously select 200 terms relevant to the medical field for each language, covering areas such as medicine, pharmacy, and medical biology \chaoyi{need a supple table to list the 200 terms} \pengcheng{200 each 6 languages=1200 terms}. Then, for sentences in languages that use spaces to separate words, we conduct word segmentation followed by keyword matching. For languages that do not use spaces for word separation, we proceed directly with keyword matching.
Utilizing the matching results, we establish two principal metrics:
\chaoyi{can we add a pseudo code to explain how a sentence is determined as filtered or left.}\pengcheng{Done}

\begin{algorithm}
\caption{Determining Medical-Related Text Samples}
\begin{algorithmic}
\State \textbf{Input:} Text $T$, Set of keywords $K$%, Language type $Lang$
\State \textbf{Output:} True or False
\State Define $T_C$ as threshold for $MKC$ and $T_D$ for $DENS$
% \If{$Lang$ = "Space Delimited"}
%     \State Segment $T$ into words based on spaces
% \EndIf
\State Initialize $K_U= \emptyset$
\State Initialize total keyword length $totalLen \gets 0$
\For{each word $t$ in $T$}
    \If{$t \in K$}
        \State Increment $totalLen$ by $len(t)$
        \If{$t \notin K_U$}
            \State Add $t$ to $K_U$
        \EndIf
    \EndIf
\EndFor
\State Calculate $MKC$ and $DENS$
\If{$MKC > T_C$ \textbf{and} $DENS > T_D$}
    \State \Return True %\Comment{Text is considered medical-related}
\Else
    \State \Return False %\Comment{Text is not considered medical-related}
\EndIf
\end{algorithmic}
\end{algorithm}

% It is important to recognize that languages similar to English use spaces to delineate words, whereas languages akin to Chinese do not. This distinction requires customized matching strategies for each language group. For languages that do not use spaces for word separation, we implement a direct matching technique to identify keywords within the text. Conversely, for languages that utilize spaces, we first segment the text into individual words based on spaces, convert these words to lowercase, and subsequently perform keyword matching.
% Then, utilizing these terms, we establish two principal metrics:

\vspace{3pt}
\noindent \textbf{Medical Keyword Count.} Medical Keyword Count quantifies the number of unique medical keywords in a text. Let \(K\) be the set of a priori keywords representing medical terms of interest, and let \(T\) denote the entire text under analysis. The set of unique keywords appearing in the text can be formulated as \(K_U = \{k \mid k \in T \wedge k \in K\}\). The Medical Keyword Count (MKC) is then defined as \(MKC = |K_U|\), where \(|\cdot|\) denotes the cardinality of the set. \chaoyi{give a formulation to explain this metric.}\pengcheng{Done}

\vspace{3pt}
\noindent \textbf{Keyword Density.} Keyword density measures the proportion of text occupied by medical keywords relative to the total text length. This metric is instrumental in identifying texts that, despite their length, only incidentally include medical terms. Let \(len(T)\) denote the total number of characters in the text \(T\), and \(occ(t, T)\) denote the occurrence times of word \(t\) in \(T\). The keyword density, denoted as \(DENS\), can be formulated as:
\[DENS = \frac{\sum_{k \in K} len(k) \cdot occ(k, T)}{len(T)}\]
\chaoyi{add equalization}\pengcheng{Done}

% \item \textbf} quantifies the number of unique medical keywords in a text. It's a threshold which reflects the extent of keyword coverage and the breadth of the medical field, thus distinguishing texts that are predominantly medical in nature from those that sporadically mention medical terms. Our analysis suggests that an ideal threshold lies between 4 and 5. Detailed threshold settings can be found in Table~\ref{tab:filtering_params_setting}.
    
    % \item KW\_DENS(Keyword Density) assesses the ratio of the length of the mentioned keywords to the entire text length. It helps in excluding instances where extensive texts inadvertently contain medical keywords. Our findings suggest that an effective threshold is approximately 1\%, a relatively stringent criterion. Given the immense volume of Common Crawl data, we prioritize data quality over quantity.

%     \item KW\_DENS (Keyword Density) measures the proportion of text occupied by medical keywords relative to the total text length. This metric is instrumental in identifying texts that, despite their length, only incidentally include medical terms. Our research indicates that a threshold of approximately 4\% serves as an effective filter. Considering the vast dataset from Common Crawl, our approach emphasizes the importance of data quality over quantity.
% \end{itemize}

% a method which computationally efficient given the sheer volume of data. This straightforward, rule-based approach begin with the compilation of a list of frequently used medical terms. Recognizing the linguistic nuances present across different languages, we meticulously select 200 terms relevant to the medical field for each language, covering areas such as medicine, pharmacy, and medical biology. Utilizing these terms, we establish two principal metrics:

% \begin{itemize}
%     % \item MEDKW\_CNT(Medical Keyword count) signifies the count of unique medical keywords present in a text. An appropriately set threshold aids in discerning if a text predominantly concentrates on medical subjects. The threshold setting should reflect the keyword coverage and the scope of the medical field, differentiating between texts predominantly about medical topics and those merely mentioning medical terms sporadically. Our evaluation indicates that an optimal threshold ranges between 4-5, varying across different languages. Detailed settings are provided in table~\ref{tab:filtering_params_setting}.

%     \item MEDKW\_CNT (Medical Keyword Count) quantifies the number of unique medical keywords in a text. It's a threshold which reflects the extent of keyword coverage and the breadth of the medical field, thus distinguishing texts that are predominantly medical in nature from those that sporadically mention medical terms. Our analysis suggests that an ideal threshold lies between 4 and 5. Detailed threshold settings can be found in Table~\ref{tab:filtering_params_setting}.
    
%     % \item KW\_DENS(Keyword Density) assesses the ratio of the length of the mentioned keywords to the entire text length. It helps in excluding instances where extensive texts inadvertently contain medical keywords. Our findings suggest that an effective threshold is approximately 1\%, a relatively stringent criterion. Given the immense volume of Common Crawl data, we prioritize data quality over quantity.

%     \item KW\_DENS (Keyword Density) measures the proportion of text occupied by medical keywords relative to the total text length. This metric is instrumental in identifying texts that, despite their length, only incidentally include medical terms. Our research indicates that a threshold of approximately 4\% serves as an effective filter. Considering the vast dataset from Common Crawl, our approach emphasizes the importance of data quality over quantity.
% \end{itemize}

% Notice that languages akin to English utilize spaces for word separation, while Chinese-like languages do not. This necessitates tailored matching strategies for these language groups. For Chinese-like languages, we employ a straightforward matching technique to ascertain the presence of keywords in the text. In contrast, for English-like languages, we segment the text into individual words based on spaces, convert them to lowercase, and then perform keyword matching.

With the two metrics, we straightforwardly set a threshold bar to perform filtering per sentence, which is easy but computationally efficient and suitable for filtering such a large-scale database.
To control the filtering quality, we randomly sampled $100$ left sentences per language, and on average, \chaoyi{98\%} sentences are manually checked as medical-related. The final threshold and filtering ratios are listed in Table~\ref{tab:filtering_params_setting}.    


\begin{table}[!htb]
\centering
\footnotesize
\tabcolsep=0.1cm
   \vspace{10pt}
    \caption{Parameter Settings for Data Filtering. Given the extensive dataset within CulturaX, the configuration of filtering parameters is designed to prioritize quality over quantity.  MKC refers to the Medical Keyword Count metric, DENS stands for the Keyword Density metric, FR signifies the proportion of the remaining text relative to the entire corpus, and tokens represent for the amount of medical corpus left  after filtering. \chaoyi{add a column about exact left token per language.}\pengcheng{Done}}
    \label{tab:filtering_params_setting}
   \begin{tabular}{ccc|cc}
        \toprule
        Language & MKC &DENS&FR&tokens\\
        \toprule
        English &5&4\%&2.29\%&6.56B\\
        Spanish &4&4\%&0.92\%&3.98B\\
        French  &4&4\%&0.50\%&1.90B\\
        Russian &4&2\%&0.48\%&1.29B\\
        Chinese &5&5\%&1.33\%&3.34B\\
        Japanese&5&5\%&1.13\%&1.93B\\
        \midrule
    \end{tabular}
\vspace{4pt}
 % \vspace{-0.8cm}
\end{table}

\subsubsection{OCR-based Data}
% Medical textbooks are a treasure trove of comprehensive medical knowledge. Their rigorous publication process further assures the quality of the content, making them a high0quality resource for medical corpus. With the advent of the internet, a vast array of medical books, often subject to varying copyright policies across countries, has become accessible. We have amassed a collection of over 20,000 books, some freely downloaded from various online sources. For those not available online, we compiled a list of titles and purchased the corresponding eBooks following \cite{PMC-LLAMA}. Our research indicates that English and Spanish medical ebooks are relatively more accessible, whereas Japanese ebooks are often heavily guarded by stringent copyright laws, posing challenges in their online acquisition. Based on these ebooks, our aim is to extract a substantial and high-quality medical corpus.
In addition to filtering from the general corpus, we also collect dozens of medical textbooks. Due to this content is stored in commonly ``PDF'' format, regular crawls may fail to catch these while, indeed, medical textbooks represent a rich repository of extensive medical knowledge, underscored by a rigorous publication process that ensures content quality. 

We have curated a collection exceeding 20,000 books, leveraging online platforms for free downloads wherever possible~\chaoyi{need a table in supplementary to list out the websites}\pengcheng{Done}. For texts not available digitally, we compiled a list of titles and bought them, in line with the methodology outlined in PMC-LLaMA~\cite{PMC-LLAMA}.  % Our investigation reveals that English and Spanish medical eBooks are more readily accessible, in contrast to Japanese eBooks, which are often encumbered by strict copyright regulations, thus complicating their digital procurement. Drawing from this collection, our objective is to distill a substantial and high-quality medical corpus

% However, a significant challenge arises as most eBooks are available in image-based PDF formats, which are not readily conducive to text parsing. To address this, we employed Optical Character Recognition (OCR), specifically choosing the ppocr tool for its support of multiple languages. The OCR process outputs a list containing the coordinates and content of each text box, which we then systematically arrange from left to right and top to bottom. During our analysis, we encountered books with right-to-left writing or dual-column layouts. Given their rarity, we did not implement specialized processing for these formats. Lastly, to maintain focus on the substantive content, we eliminated non-essential pages such as covers, tables of contents, and epilogues, relying on their page numbers for identification.

The main challenge for processing such data is that most eBooks are in image-based ``PDF'' formats. To overcome this issue, we utilized Optical Character Recognition (OCR) technology. Specifically, we select the PaddleOCR\chaoyi{whats this? write down the python package name and introduce it more formally} tool for its proficiency in handling multiple languages. The OCR process generates a list detailing the coordinates and content of each text box, which is then organized in a left-to-right and top-to-bottom sequence. Throughout our analysis, we encountered instances of books formatted with right-to-left writing or dual-column layouts. Due to their infrequent occurrence, we opted not to develop specialized processing techniques for these formats. Furthermore, to ensure a focus on medical content, we excluded non-essential pages, such as covers, tables of contents, and epilogues, identifying them by their page numbers for removal. We have to emphasize that due to the varying degrees of openness regarding books across different countries, the amount of corpus obtained via OCR varying a lot for different languages. Quantitatively, we finally collect 4B tokens for English, 1.1B tokens for Chinese, 0.4B tokens for Russian and 0.3B tokens for French.\chaoyi{list out how many tokens are collected in total and per language}\pengcheng{Done}

\subsubsection{Crawled-based Data}

Considering that filtering-based data are based on CommonCrawl, which is randomly scratched and untraceable, to avoid missing some important medical knowledge websites, we further crawled some famous and critical medical-related websites as compensatory. We focus on three categories of websites. Firstly, we target medical encyclopedias, which offer detailed information on diseases and drugs. While this data is of exceptional quality, it is often limited in quantity and subject to stringent access controls. Secondly, we source content from medical consultation platforms and popular science articles about medicine. These sources, though less technical, provide a wealth of knowledge on medical common sense. Lastly, we expand our data collection to include medical news websites, which allow us to gather a larger volume of unrestricted data and incorporate timely information into our model. This strategy enhanced the model's ability to understand and respond to current medical events and trends. Collecting data from these varied websites, we compile a comprehensive and diverse medical corpus, encompassing in-depth professional medical knowledge as well as a broad spectrum of general medical information and up-to-date industry insights. The detailed websites are listed in \chaoyi{list them in supplementary} \pengcheng{Done}and as a result we get 0.1B tokens for Japanese, 0.05B tokens for Spanish and 0.1M tokens for French.\chaoyi{similarly, write down the exact number.}\pengcheng{Done}

\subsubsection{Open-source Dataset}

Except for the above newly collected data, we also leverage many existing open-source datasets consisting of lots of domain knowledge, merging into our corpus. Specifically, we utilized the following three datasets: Wikipedia~\cite{wikidump}, Baidu Baike~\cite{baidu_baike}, and UFAL Medical Corpus~\cite{ufal_medical_corpus}. For Wikipedia and Baidu Baike, we employ the same filtering methodology outlined in Section~\ref{sec:filtering_based_data} to extract the medical domain corpus, while for UFAL, we use it directly as it is a medical corpus designed for translation tasks.
% \chaoyi{We can also add some translated texts though I think it is not so good but anyway if we have we can do ablation on it and release them in separate dir.}

\subsubsection{Distribution Analysis}

% In this subsection, we perform an in-depth analysis of MMedC. The dataset distribution across different languages is detailed in table~\ref{tab:data_distribution}. As our objective in constructing MMedC was to create a high-quality, multilingual medical corpus, we attempt to achieve a balance between the amount of corpus in different languages via collecting data from 4 sources.  
From the above four sources, we collect \chaoyi{25.5}B tokens in total, termed as Multilingual Medical Corpus~(MMedC). In this section, we conduct a comprehensive analysis on it, with the distribution of the dataset across various languages presented in Table~\ref{tab:data_distribution}. Intuitively, we aim to balance the corpus volume across different languages by seeking data from various sources. Furthermore, we categorize the MMedC into two segments: high-quality data and unsure-quality data. We define \chaoyi{data sourcing from books, websites and carefully constructed datasets } as high-quality data, while \chaoyi{data sourcing from CommonCrawl} as unsure-quality data. We make this distinction because the former mostly are directly collected from strictly human-verification medical-related media and the latter mostly rely on auto-filtering progresses and are not surely medical-related. In our later ablation study, we will carefully discuss whether the unsure-quality data is clean and valuable enough to be added into LLM pre-training.

% \chaoyi{Totally miss the following sentences...}
% This bifurcation is crucial for evaluating the efficacy of medical data derived from CommonCrawl, which has not been subjected to human verification, in contributing to the pretraining phase of the language model. This differentiation highlights the potential benefits of utilizing large, unverified datasets in the enhancement of LLMs' domain knowledge. Notably, the unsure-quality data demonstrates its value in our ablation study.

% Additionally, we divided MMedC into two categories: high-quality data and unsure-quality data. This separation is pivotal for assessing whether medical data extracted from CommonCrawl, which hasn't undergone human verification, can contribute effectively to the language model during its pretraining phase. This distinction underline the potential of leveraging large, unverified datasets to enhance language model training, particularly in specialized fields such as medical informatics. The unsure-quality data proves efficient in the ablation study.


\subsubsection{Pre-training with MMedC}
With MMedC, we can simply further pre-train any existing LLM on it. 
We simply adopt the auto-regressive loss as GPT~\cite{openai2023gpt4}. Specifically, we treat medical text as a sequence of tokens, denoted as $X=\{x_1, x_2, \dots, x_N\}$, where each $x_i$ is a text token and $N$ represents the total length of the sequence. 
Auto-regressive language models predict the following words solely on the preceding sequence. These models mask all tokens following the token to be predicted. For a token \( x_i \) to be predicted, the optimization objective is:
\begin{equation}
    L(\phi)=-\sum \log(\Phi(x_i|x_{<i}))
\end{equation}
We denote the new models pre-trained on MMedC as MMedLM and in specific experiments, we will further distinguish what existing LLMs it is initialized with.

\begin{table}[!htb]
\centering
\footnotesize
\tabcolsep=0.1cm
   \vspace{10pt}
    \caption{Corpus statistics. The Multilingual Medical Corpus (MMedC) boasts a substantial size of 105GB, comprising over 25 billion tokens. The dataset is categorized into several types by sources: FData represents filtering-based data, OCRData denotes Optical Character Recognition (OCR)-based data, CData refers to data obtained through web crawling, and OSData signifies data from open-source datasets. Furthermore, we distinguish between HQData (high-quality data) that has undergone human verification, and UQData (unsure-quality data), which has not. The TotAmt (Total Amount) quantifies the total token count for each language, with 'Billion tokens' serving as the unit of measurement. \chaoyi{em, why this table does not fill the page from left to right... Noe this is so wired.} }
    \label{tab:data_distribution}
   \begin{tabular}{cc|cccc|cc|c}
    \toprule
    Language & Family& FData& OCRData& CData& OSData& HQData&UQData &TotAmt\\
    \toprule
    English	&Indo-European& 6.56&4.00&0.00&0.00&4.00&6.56&10.56\\
    Spanish	&Indo-European&	3.98&0.31&0.05&0.02&0.37&3.98&4.35\\
    French	&Indo-European&	1.90&0.02&0.00&0.17&0.20&1.90&2.10\\
    Russian	&Indo-European&	1.29&0.40&0.00&0.00&0.40&1.29&1.69\\
    \midrule
    Chinese	&Sino-Tibetan&	3.34&1.21&0.00&0.19&1.40&3.34&4.74\\
    Japaneses&Sino-Tibetan&	1.93&0.00&0.10&0.01&0.12&1.93&2.05\\
    \midrule
    \end{tabular}
  \vspace{4pt}
 % \vspace{-0.8cm}
\end{table}

\subsection{Comprehensive Multilingual Medical Benchmark}
\label{sec:MMedB}
% To have a comprehensive evaluation of a model's performance in the medical domain across various languages, we introduce \textbf{MMedB}, a multilingual Medical Benchmark encompassing six primary languages. We first collected existing medical QA evaluation benchmarks for each language. Subsequently, we enrich the dataseted by incorporating rationales generated by GPT-4 and then do human checking, facilitating a more thorough evaluation of the model's comprehension capabilities. Finally, we undertake an exhaustive analysis of MMedB's characteristics.
Beyond MMedC, we also collect a new comprehensive Multilingual Medical Benchmark spanning 6 principal languages, namely \textbf{MMedB}, to conduct a thorough evaluation of a model's performance in the medical domain across diverse languages

Specifically, we started by collecting existing medical question-answering~(QA) benchmarks for each language while most QA benchmarks are all in the mutiple-choice format which lacks further evaluation on the critical long sentence reasoning ability. Thus, then we expand these multi-choice QA with corresponding explanations using GPT-4, followed by strict human verification to ensure the correctness of contents, providing a deeper insight into the model's understanding and reasoning abilities. Lastly, we also undertake an exhaustive analysis of MMedB's characteristics.

\subsubsection{Multilingual Medical QA data Collection}
% \chaoyi{Whether some benchmarks have detailed analysis? we can construct a extra rationale version of the Benchmarks and check the model's ability in generate rationale. For the dataset with no analysis we can use GPT-4 to add and do manually check in paper.}\pengcheng{Done}

% \chaoyi{And for a medical paper, if possible we need to track the patient related in the question distribution on the Benchmark, e.g, female/male, age and Adult/Child, human system and if some aspects are limited or missed we can use GPT-4 to auto-generate use our pre-train corpus or translate from other language which I think can greatly enhance our contribution on the benchmark. Also how much AvG tokens for different language in question /in context/ in answer and a question type set should be defined and statisticed, maybe check the pubmedQA and USMLe original paper to see how they demonstrate the dataset.}\pengcheng{Done}
% \chaoyi{furthermore, if some tailed language do not have benchmark we can also auto-generate some questions using GPT-4 or translate then manual check.}

% Currently ,the most efficient quantitative metrics for evaluation the performance of LLMs is utilizing multiple-choice question, as using the question and options as query. while expecting the model output the right answer index. This straightforward and objective measure using accuracy as its metric. However, current medical multiple-choice QA benchmarks, which are predominantly monolingual, fail to meet the multilingual demands of the medical field. To address this gap, we have collected a representative multiple-choice question indicator for each of the six languages under consideration. They are as follows

Currently, the most effective quantitative metric for evaluating the performance of Large Language Models (LLMs) involves the use of multiple-choice questions, wherein the question and its options are presented as a query, with the expectation that the model will output the correct answer index. This method employs accuracy as its primary metric, offering a straightforward and objective means of assessment. However, existing medical multiple-choice QA benchmarks are all monolingual, failing to meet the demand of evaluating LLMs' performance across different languages. To bridge this gap, we start by collecting various medical multiple-choice QA datasets together. The following benchmarks are considered:

\begin{itemize}
    \item \textbf{MedQA}~\cite{jin2020disease} is a collection of medical multiple-choice questions (each with four answer options) based on the USMLE examination. It encompasses data in three languages: English, Simplified Chinese, and Traditional Chinese. For our evaluation, we exclusively utilize the English and Simplified Chinese sections. The data is partitioned in accordance with official guidelines. %For the English section, the training set comprises 10,178 samples, the validation set includes 1,272 samples, and the test set consists of 1,273 samples. As for the Simplified Chinese dataset, the training set comprises 27,400 samples, the validation set contains 3,425 samples, and the test set comprises 3,426 samples.
    \item \textbf{lgakuQA}~\cite{jpn-med-exam_gpt4} is a Japanese medical multiple-choice question dataset, which comes from Japanese medical licensing examinations from the past five years (2018-2022). Since there is no official data division, we randomly divide the data, and get 1,590 training samples, 199 validation samples, and 199 test samples.
    \item \textbf{FrenchMedMCQA}~\cite{labrak:hal-03824241} is a French medical multiple-choice question dataset, which comes from real exams of the French medical specialization diploma in pharmacy. The data is divided according to the official way. %there are 2,171 training samples, 312 validation samples, and 622 test samples.
    \item \textbf{RuMedDaNet}~\cite{blinov2022rumedbench} is a Russian medical judgment question dataset, which we process into a binary-choice question format. The data is divided according to the official way. %there are 1,052 training samples, 256 validation samples, and 256 test samples.
    \item \textbf{Head-QA}~\cite{vilares-gomez-rodriguez-2019-head} is a Spanish multiple-choice question dataset. Questions come from exams to access a specialized position in the Spanish healthcare system. The data is divided according to the official way. % and there are 2,657 training samples, 1,366 validation samples, and 2,742 test samples.
\end{itemize}

As a result, we collect \chaoyi{53566} QA pairs in total, and we split them following the official way. Otherwise we split them in\chaoyi{8:1:1} for training, validating and testing respectively.

\subsubsection{Rationale Generation}
% Despite Accuracy is an straightforward metric, it fails when the model just happens to output the correct answer without having the relevant knowledge or reasoning, as shown in Figure~\ref{fig:case5}. To avoid this from happening, we also need to evaluate the reasoning process by which the model produces the answer. Based on the multiple-choice QA data we have collected, we further give each question a reason for choosing the right option. During evaluation, we need model to generate the rationale of its choice, thus giving an insight into how the model comes out he result. 

Although the accuracy of multiple-choice is a straightforward and accurate metric, it fails to evaluate the reasoning and long sentence generation abilities of LLMs, which is critical for clinical usage. Thus, leveraging the multiple-choice QA data we have collected, we further augment each question with a justification for selecting the correct option. During the evaluation phase, we require the model to articulate the rationale behind its choice, thereby offering insights into the model's reasoning capabilities.

In detail, given GPT-4's demonstrated capability to outperform human experts by providing detailed explanations in Chain of Thought (CoT) experiments~\cite{kung2023performance}, we utilize GPT-4 to generate rationales for our dataset. To guarantee the quality of these explanations, we subsequently perform human verification. Specifically, we input the question, the options, and the correct choice into GPT-4, instructing it to generate a detailed rationale for selecting a particular option. The instructions provided to GPT-4 are as follows:
\begin{mdframed}[backgroundcolor=gray!20]
You're a \{language\} doctor. Analyze the reasons behind choosing this particular option in 100 words for the following question in \{language\}.
\end{mdframed}
Following the generation of rationales by GPT-4, we conducted a meticulous manual review to assess their quality. Our evaluation criteria are dual-focused: firstly, the explanation provided by GPT-4 had to be consistent with the established correct answer for the question; secondly, it's required to articulate the logic underpinning the answer, rather than merely replicating it. Note that considering the cost of human checks, this will only be performed on our partial testing set. Specifically, we randomly selected 200 samples from the test set of each language to form a new rationale testing split. Then we shuffled and distributed among three annotators for manual verification. Annotators were tasked with categorizing each rationale as either qualified or unqualified based on the aforementioned criteria. Remarkably, we observed that 94.7\% of the rationales generated by GPT-4 adhered to our standards, underscoring the high quality of the explanations. During the final evaluation phase, the calculation of rationale similarity was exclusively applied to these human-verified passed samples.

Finally, we get \chaoyi{1136} human-checked samples for rationale evaluation and compensate the former split \chaoyi{45048} training QA pairs with auto-generated rationale sentences. Given a language model, it can use our training set to further fine-tune and then be evaluated or directly evaluated on the rationale and choice testing sets.
% In our empirical validation, we scrutinized the explanations generated by GPT-4 through manual inspections. From each of the six benchmarks, we randomly chose 200 samples, resulting in a total of 1,200 samples for evaluation. The criteria for this test were twofold: firstly, the explanation provided by GPT-4 must align with the standard answer to the given question; secondly, it should elucidate the reasoning behind the answer rather than merely echoing it. Our analysis revealed that 94.7\% of these explanations met our criteria for validity. It is pertinent to mention that although GPT-4 was employed to generate explanations for all samples across these benchmarks, our assessment was limited to the manually inspected samples.

\subsubsection{Characteristics}
% We conduct statistics from various dimensions on MMedB. We first analyse the basic characteristics of the data, as shown in Table~\ref{tab:basic_statistics}. In addition, statistics on the themes of the samples were also performed. We use GPT4 to classify the topics of samples in the test set. The instructions used by GPT4 are as follows:

We perform multi-dimensional statistical analyses on MMedB to thoroughly understand its composition. Initially, we examine the fundamental characteristics of the dataset, with the findings detailed in Table~\ref{tab:basic_statistics}. Furthermore, we explore the thematic distribution of the samples. For this purpose, we employ GPT-4 to categorize the topics within the test set. The instructions provided to GPT-4 for topic classification are outlined as follows:
\begin{mdframed}[backgroundcolor=gray!20]
You're a \{language\} doctor, choose one subject out of \{medical\_subjects\_string\}, which is most relevant to the following question. 
\end{mdframed}
% Sometimes GPT4 gives confusing classification results, such as not in medical\_subjects\_string. In this case, we will let GPT4 retry classification 4 times. If the classification result that meets the specification cannot be given, the category of the sample will be classified as None. Considering that this situation is very rare, it will not have a big impact on the statistics. The results in fig~\ref{fig:topics_distribution} indicate that our multilingual benchmark comprehensively covers multiple facets of the medical domain, ranging from basic medicine and clinical medicine to pharmacology and public health. It primarily focuses on areas such as Biochemistry in basic medicine and Internal Medicine in clinical medicine. Consequently, this benchmark serves as a thorough measure of a model's ability to recognize and understand various aspects within the medical field.
At times, GPT-4 may yield ambiguous classification outcomes, such as those not aligning with predefined medical subjects. In these instances, we prompt GPT-4 to reattempt the classification up to four times. Should it fail to produce a categorization that adheres to our criteria, we assign the sample's category as 'None.' Given the rarity of such occurrences, their impact on the overall statistics is minimal. The distribution illustrated in Figure~\ref{fig:topics_distribution} demonstrates that our multilingual benchmark extensively spans various sectors of the medical field, from basic and clinical medicine to pharmacology and public health, with a pronounced emphasis on areas like Biochemistry within basic medicine and Internal Medicine in clinical settings. This comprehensive coverage ensures the benchmark effectively evaluates a model's proficiency in recognizing and understanding diverse medical topics.

\begin{table}[!htb]
\centering
\footnotesize
\tabcolsep=0.1cm
   \vspace{10pt}
    \caption{Overall statistics of MMedB. The token number is got with the help of tokenizer used by multilingual-bert. }
    \label{tab:basic_statistics}
   \begin{tabular}{lcc}
    \toprule
    statistics & Trainset & Testset\\
    \toprule
    Number of QA paris&45048 &8518\\
    % \midrule
    % Prop. of A(\%)&23.4 &24.1\\
    % Prop. of B(\%)&25.6 &25.8\\
    % Prop. of C(\%)&24.7 &25.2\\
    % Prop. of D(\%)&22.7 &22.1\\
    % Prop. of E(\%)&3.6  &2.8 \\
    \midrule
    Prop. of single-choice(\%)&91.7 &90.4\\
    Prop. of muti-choice(\%)  &8.3  &9.6\\
    \midrule
    Avg. question tokens &76.3  &63.9  \\
    Avg. option tokens   &40.3  &45.7  \\
    Avg. rationale tokens&210.2 &192.8 \\
    \midrule
    \end{tabular}
  \vspace{4pt}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/topics_distribution.pdf}
    \caption{The topics in MMedB cover a wide range of medical aspects, ranging from general and specialized medicine to basic medical sciences. This allows MedQA to comprehensively measure the performance of medical models.}
    \vspace{-10pt}
    \label{fig:topics_distribution}
\end{figure}




% \subsection{Medical knowledge injection procedure}
% We use InternLM-7b~\cite{2023internlm} as our base model, which is an open-source LLM with good multilingual understanding ability developed by Shanghai AI Lab. We pretrain it on the pretraining dataset we constructed previously. The optimization objective is the same in autoregressive generation task, which was first proposed in ~\cite{radford2019language}. During the training process, the maximum context length is set to 2048, and the global batch size is set to 128. The model is optimized using the AdamW optimizer, with a learning rate of 2e-5. Due to the model having too many parameters to fit on one GPU, we use the FSDP strategy to distribute the model to multiple GPU cards, and use the BF16 data type and gradient checkpointing technique to save memory. The model is trained for 5 epochs on 8 A100 GPUs for about 11 hours. We call the model medical foundation model.


% \subsection{Evaluation settings}
% We mainly use two methods for evaluation, which are fine-tuning evaluation and zero-shot evaluation.
% \begin{itemize}
%     \item \textbf{Finetuning evaluation} requires training the model on the trainset of the benchmark, and then evaluating it on the testset. We adopted this method for all models with open-source weights, to achieve a more fair comparison.
%     \item \textbf{Zero-shot evaluation} does not require training the model, but rather designing a prompt to allow the model to make the correct choice. For all the models with non-open-source weights, we used this method for evaluation, such as GPT-3.5, GPT-4, etc.
% \end{itemize}



==> content_acl/04_Experiment_and_Results.tex <==

\section{Experiment and Results}
% In this section, we firstly detailed the performance of various leading large language models on the MMedB. Subsequently, we conduct human rating to give a more convincing evaluation of the quality of rationale generating by LLMs. Finally, we engaged in a series of ablation experiments designed to analyze the influence of each stage in the enhancement of medical knowledge. 

In this section, we first present the implementation details and evaluation metrics. Then we benchmark various leading existing LLMs on MMedB together with the ones further pre-trained on our MMedC to show the superior of our new corpus. Lastly, we conduct a series of ablation studies to examine the effect of each phase in data construction.

\subsection{Implementation Details}
\pengcheng{pretraining and finetuning details are currently shown in Appendix.}
\subsubsection{Pre-training}
\chaoyi{add details, like bs, lr, accelerate methodology...}  

\subsubsection{Fine-tuning} Considering the multilingual medical QA scenario is quite a challenging case for most existing LLMs~(nearly random for most open-source LLMs zero-shotly), we choose to further fine-tune them on our MMedB training set and then evaluate instead of directly evaluating using suitable instruction.   \chaoyi{add details, like bs, lr, accelerate methodology...}. But for close-source models that can't be trained, like GPT-4, we can only evaluate it in a zero-shot manner without further fine-tuning.

\subsection{Metrics}
\chaoyi{ACC BLEU Rouge and human rating. Introduce metrics here instead of separating them in the following discussion.}\pengcheng{Done}
% In order to evaluate the performance of LLMs, we calculate Accuracy and Rationale Similarity. For Accuracy, it's easy to measure as the LLM has learnt to output the results in the format of the template. Nonetheless, it's not easy to measure the Rationale Similarity as it is a general problem in NLP domain. Here, we first tried BLEU and ROUGE, 2 classic text similarity method based on n-grams to measure sentence similarity. Then we tried bert-score, which use a pretrained bert to extract high-level semantic features, then similarity is calculated by cosine similarity. Finally, we choose some representative LLMs and conduct GPT-4 Rating and Human Rating to have a better view of if these automatic metric can reflect the performance of LLMs. Among them, the BLEU and Rouge are implemented by NLTK and ROUGE libraries respectively, and bert-score is implemented by its official repository.

To evaluate the performance of LLMs, we employ two metrics: Accuracy and Rationale Similarity. Measuring Accuracy is straightforward, as the LLM can generate outputs following a specific template. However, assessing Rationale Similarity presents a more complex challenge, typical within the NLP domain. Initially, we applied two classical text similarity methods, BLEU\cite{papineni-etal-2002-bleu} and ROUGE\cite{lin-2004-rouge}, which rely on n-grams to evaluate sentence similarity. Subsequently, we explored bert-score\cite{zhang2020bertscore}, leveraging a pretrained BERT model to extract high-level semantic features, with similarity assessed via cosine similarity. 

To gain comprehensive insights into whether these automated metrics reflect LLM performance, we select several representative LLMs, and conduct GPT-4 Rating\cite{zheng2023judging} and Human Rating. Among them, the BLEU and ROUGE are implemented by NLTK and ROUGE libraries respectively, while bert-score utilizes its official repository.

\subsection{Comparison on MMedB}

As shown in Table~\ref{tab:benchmark_comparison}, We compare our models with other SOTA models on MMedB with different metrics for two aspects, \emph{i.e.}, multiple-choice, and rationale.

\chaoyi{modify the following paragraph into the following logic. Separate out the metric introduction.}
\subsubsection{Comparison on Multiple-choice}

\subsubsection{Comparison on Rationale}
\chaoyi{rememeber mention the human rating consistency}

Among them, the BLEU and Rouge are implemented by NLTK and ROUGE libraries respectively. In open-source models, we can observe that medical models based on LLaMA have achieved commendable results in English benchmarks. However, their performance in other languages, particularly in Chinese and Japanese, is not as impressive, and often falling short of the capabilities of general-purpose multilingual models. Yet, these general-purpose models, not being specific to the medical field, lack certain medical knowledge. By employing our method to pretrain multilingual models on MMedC, we infuse medical knowledge from various languages into the model. This approach significantly enhances the model's performance across each language, letting InternLM, a 7B model has much better performance on MMedB than GPT-3.5.
% \chaoyi{need to add a medical multi-linguish BERT-wise model (I don't know which one is good, maybe you should find one) to polish the table. and somehow highlight how different models are tested finetuned or zero-shot. Also benchmark the method that simply expand the token list of LLaMA-2 and then finetune on our benchmarks then test.}
\begin{table*}[!htb]
\centering
\begin{threeparttable}[b]
\footnotesize
\tabcolsep=0.1cm
   \vspace{10pt}
    \caption{Evaluation on MMedB. We presented a two-dimensional analysis of the models' performance. Firstly, we report their accuracy on the MMedB multiple-choice questions, offering a breakdown of each model's accuracy across various languages, with AVG denoting the mean score over six languages. Secondly, MMedB provides rationales that serve as a benchmark for gauging the models' understanding of medical queries. To assess this aspect, we employed two evaluation metrics, BLEU and Rouge, and computed the average scores for each language to provide a comprehensive overview of the models' interpretive capabilities.}
    \label{tab:benchmark_comparison}
   \begin{tabular}{c|cccccc|ccc}
    \toprule
    Method & MedQA & USMLE-zh& lgakuQA & FrenchMedQA & RuMedDaNet& Head-QA &AVG & BLEU&Rouge\\ \toprule
    GPT-3.5     &62.6 &50.64 &31.66 &29.74 &69.53 &66.81 &51.83&0.073&0.284\\
    GPT-4        &78.0&75.1&72.9&56.6&83.6&85.7&74.27&/&/\\
    \midrule
    BLOOM-7b   &43.28 &58.06 &32.66 &26.37 &62.89 &47.34 &45.1 &0.117 &0.324\\
    InternLM-7b &44.07 &64.62 &37.19 &24.92 &58.2 &44.97 &45.67 &0.114 &0.321\\
    Llama\ 2     &43.36 &50.29 &25.13 &20.90 &66.80 &47.10 &42.26 &0.118 &0.324\\
    MedAlpaca  &46.74 &44.80 &29.64 &21.06 &59.38 &45.00 &41.11 &0.119 &0.327\\
    ChatDoctor  &43.52 &43.26 &25.63 &18.81 &62.5 &43.44&39.53&	0.115&	0.325\\
    PMC-LLaMA   &47.53 &42.44 &24.12 &20.74 &62.11 &43.29 &40.04&0.118&	0.325\\
    Mistral    &61.74 &71.1 &44.72 &48.71 &74.22 &63.86 &60.73& 0.125 &	 - \\
    InternLM\ 2   &57.27 &77.55 &47.74 &41.00 &68.36 &59.59 &58.59& 0.139 &	 - \\
    \midrule
    MMedLM        &49.88&70.49&46.23&36.66&72.27&54.52&55.01&0.132&0.341\\
    MMedLM\ 2       &61.74&80.01&61.81&52.09&80.47&67.65&67.30& 0.159 & -\\
    \midrule
    \end{tabular}
  \end{threeparttable}
  \vspace{4pt}
     % \vspace{-0.8cm}
\end{table*}





\subsection{Human Rating}
To have a better evaluation of the rationale generating by the LLMs, we incorporated human ratings. From MMedB, we randomly selected 50 samples for each language, ensuring these samples had previously verified rationales. We then chose the generated outcomes from six representative models for these samples. The order of the samples was randomized before distribution to five medical students for assessment. These annotators were instructed to rank the outputs from the six models based on three criteria: accuracy, reasoning ability, and the model's internal knowledge. Scoring was assigned based on their ranking, with the top rank receiving a score of 6 and the bottom rank a score of 1. This approach quantified the output quality of each model. Parallel to ~\cite{zheng2023judging}, we utilized GPT-4 to rank the model outputs as well. Further details regarding the annotation process are available in the appendix.

The Figure~\ref{fig:ratings_comparison} visually demonstrates the comparison of various models across different metrics. It is evident that, despite some variations under different metrics, the MMedLM enhanced with domain knowledge consistently achieves the best results. Detailed results for each language and each model are presented in the appendix. Moreover, due to observed discrepancies in the ranking of similarly scored models under different metrics, appendix B includes an analysis of the relationship between automated and human evaluation metrics.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ratings_comparison.png}
    \caption{Comparative analysis of model ratings. BLEU scores, presented as absolute values, are referenced using the left-hand scale. In contrast, the other two evaluation methods initially rank the models' outputs by quality, subsequently converting these rankings into relative scores, as denoted on the right-hand scale.}
    \vspace{-10pt}
    \label{fig:ratings_comparison}
\end{figure}


\subsection{Ablation Study}
\chaoyi{This section roughly seems good in logic. I may read more carefully later.}
In this section, we present more thorough ablation studies to assess the impact of different data types and training strategies on our model's performance as shown in Tab.~\ref{tab:ablation_study}.

\begin{table*}[!htb]
\centering
\begin{threeparttable}[b]
\footnotesize
\tabcolsep=0.1cm
   \vspace{10pt}
    \caption{Ablation study on MMedB. We reported all ACC, BLEU and Rouge score to give a overall knowledge of the effect of each step.}
    \label{tab:ablation_study}
   \begin{tabular}{c|cc|ccc|cc|ccc}
    \toprule
    Method & English & Multilingual& OCR & webcrawl &Filtering& QA Answer &Rational&ACC & BLEU&Rouge\\ 
    \toprule
    Baseline(InternLM)&\ding{55}&\ding{55}&\ding{55}&\ding{55}&\ding{55}&\ding{52}&\ding{55}&43.33&/&/\\
    Baseline(InternLM)&\ding{55}&\ding{55}&\ding{55}&\ding{55}&\ding{55}&\ding{52}&\ding{52}&45.66&0.114&0.321\\
    \midrule
    Med-InternL$\mathrm{M}_{en}$&\ding{52}&\ding{55}&\ding{52}&\ding{52}&\ding{55}&\ding{52}&\ding{52}&47.38&0.114&0.323\\
    Med-InternL$\mathrm{M}_{ocr}$&\ding{52}&\ding{52}&\ding{52}&\ding{52}&\ding{55}&\ding{52}&\ding{52}&51.33&0.124&0.334\\
    \midrule
    Med-InternLM&\ding{52}&\ding{52}&\ding{52}&\ding{52}&\ding{52}&\ding{52}&\ding{52}&55.01&0.132&0.341\\
    \midrule
    \end{tabular}
  \end{threeparttable}
  \vspace{4pt}
     % \vspace{-0.8cm}
\end{table*}


\subsubsection{Influence of multilingual pretraining}
Current studies have shown that pretraining on medical corpus can injecting medical common sense into the LLM. However, the impact of pretraining on multilingual medical corpus remains unclear. Here we investigate whether this approach can infuse diverse medical knowledge from various languages into the model, potentially enhancing its comprehension of multilingual medical questions. 

The results show that pre-training with a multilingual medical corpus improved model performance by 1\%. This finding corroborates our assumption that such pre-training aids the model's understanding of medical questions across different languages.

\subsubsection{Efficiency of corpus filtered from general datasets}
Although the corpus filtered from CulturalX seems to be highly medical-related, there remains doubt that whether such kind of data's quality is high enough for training a model. Our study investigate into the effectiveness of medical-related corpora extracted from larger datasets like CommonCrawl on model performance. 

Due to computational resource limitations, a subset of this corpus was used, with specifics on the selection ratio provided in the Appendix. The results show that even a subset of the medical-related corpus derived from CommonCrawl proved beneficial for training the medical language model. The specific impact and methodology are detailed in the Appendix.

\subsubsection{Influence of rationale data}
Finally, beyond analysis on MMedC, we also examine whether fine-tuning the model with rationale-annotated data can directly help improve multiple-choice QA accuracy. The results of ablation study reveals that fine-tuning the model with both correct answers and their rationales leads to a 2.33\% increase in accuracy on the MultilingualMedQA Benchmark. This supports our hypothesis that rationale integration enhances the model's reasoning capabilities in medical Q\&A.


==> content_acl/05_Conclusion.tex <==

\section{Conclusion}
In this paper, we introduce an innovative pipeline for building up a new multilingual medical corpus together with a new benchmark. Specifically, we developed MMedC, a comprehensive 105GB medical corpus with 25B tokens covering 6 main languages, and MMedB, a benchmark encompassing 6 primary languages, evaluating multilingual medical LLMs both form multiple-choice and rationale abilities. In experiments, we show that by further pre-training on MMedC, our new LLM MMedLM can achieve comparable performance with strong baseline GPT-3.5, demonstrating the effectiveness of our new corpus. Our thorough ablation study also validates the effectiveness of our methodology. 
